Autoregressive Pre-Training on Pixels and Texts

The integration of visual and textual information represents a promising direction in the advancement of language models. In this paper, we explore the dual modality of language--both visual and textual--within an autoregressive framework, pre-trained on both document images and texts. Our method employs a multimodal training strategy, utilizing visual data through next patch prediction with a regression head and/or textual data through next token prediction with a classification head. We focus on understanding the interaction between these two modalities and their combined impact on model performance. Our extensive evaluation across a wide range of benchmarks shows that incorporating both visual and textual data significantly improves the performance of pixel-based language models. Remarkably, we find that a unidirectional pixel-based model trained solely on visual data can achieve comparable results to state-of-the-art bidirectional models on several language understanding tasks. This work uncovers the untapped potential of integrating visual and textual modalities for more effective language modeling. We release our code, data, and model checkpoints at \url{https://github.com/ernie-research/pixelgpt}.

==> table/analysis_mode_glue.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \begin{table*}[]
% \resizebox{\linewidth}{!}{\ttfamily
% \small
% \begin{tabular}{@{}lllllllllll@{}}
% \toprule
% \multirow{2}{*}{\textbf{Render Mode}} & \textbf{MNLI-m/mm} & \textbf{QQP} & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{STS-B} & \textbf{MRPC} & \textbf{RTE} & \textbf{WNLI} & \multirow{2}{*}{\textbf{Avg.}} \\ \cmidrule(lr){2-10}
%  & Acc & F1 & Acc & Acc & MCC & Spear. & F1 & Acc & acc &  \\ \midrule
% RGB & 79.0/78.2 & 86.0 & 85.6 & 90.1 & 35.3 & 80.3 & 84.6 & 63.9 & 59.2 & 74.2 \\
% Binary & 77.9/78.2 & 85.0 & 84.8 & 90.0 & 17.5 & 68.9 & 83.3 & 61.7 & 59.2 & 70.7 \\
% Grayscale & 78.7/78.9 & 85.1 & 85.1 & 89.8 & 34.0 & 21.0 & 83.6 & 62.1 & 60.6 & 67.9 \\ \bottomrule
% \end{tabular}
% }
% \caption{Comparison of using three different render mode to fine-tune \textbf{{\PixelGPT}} on GLUE.}
% \end{table*}

==> table/corpus_at_a_glance.tex <==
\begin{table*}[!htbp]
\centering
\captionsetup{justification=centering,singlelinecheck=false}
\resizebox{\textwidth}{!}{\ttfamily
\begin{tabular}{lcccc}
\hline
\textbf{Source} & \textbf{Type} & \textbf{Gzip files (GB)} & \textbf{Documents (millions)} & \textbf{Tokens (billions)} \\
\hline
CommonCrawl & web & 4,197 & 4,600 & 2,415 \\
C4 & web & 302 & 364 & 175 \\
peS2o & academic & 150 & 38.8 & 57 \\
The Stack & code & 319 & 236 & 430 \\
Project Gutenberg & books & 6.6 & 0.052 & 4.8 \\
Wikipedia & encyclopedic & 5.8 & 6.1 & 3.6 \\
\hline
\textbf{Total} & & 4980.4 & 5,245 & 3,084 \\
\hline
\end{tabular}%
}
\caption{The corpus at-a-glance.}
\label{tab:datasets}
\end{table*}

